Exploring the Use of Robots for Diary Studies

As interest in studying in-the-wild human-robot interaction grows, there is a need for methods to collect data over time and in naturalistic or potentially private environments. HRI researchers have increasingly used the diary method for these studies, asking study participants to self-administer a structured data collection instrument, i.e., a diary, over a period of time. Although the diary method offers a unique window into settings that researchers may not have access to, they also lack the interactivity and probing that interview-based methods offer. In this paper, we explore a novel data collection method in which a robot plays the role of an interactive diary. We developed the Diary Robot system and performed in-home deployments for a week to evaluate the feasibility and effectiveness of this approach. Using traditional text-based and audio-based diaries as benchmarks, we found that robots are able to effectively elicit the intended information. We reflect on our findings, and describe scenarios where the utilization of robots in diary studies as a data collection instrument may be especially applicable.

==> 80_backup.tex <==
20240924 - 09:24

\section{Results}
\todo{add some data points in text where appropriate}

We report results on 1. the information richness of the diary entries; 2. the system's usability; and 3. the participants' compliance in completing the study.


\subsection{Information Richness and Disclosure}
We analyzed both the diary entries that were created by the participants, and the subjective measures reported in the post-study questionnaire. We found that diary entries created by participants in the \textit{Robot Group} on average included comparable amount of information as those from the \textit{Audio Group}, with both containing more than those from the \textit{Text Group}.
% more information than those from the \textit{Text Group}. The overall information levels are comparable between entries from the \textit{Robot Group} and the \textit{Audio Group}, 
However, participants in the \textit{Robot Group} were able to achieve this level of information richness with more efficient usage of words, and on average better maintain the level of information richness over the course of the week-long study. Participants from the \textit{Robot Group} self-reported a lower level of \textit{breadth} in terms of their information disclosure, while the self-reported \textit{depth} are comparable across the three groups. While there isn't a precise mapping from the breadth and depth of disclosure to the various content analysis dimensions, this pattern is consistent with our findings that compared to those from the \textit{Audio Group}, entries from the \textit{Robot Group} included less information on activities outside of the children's bedtime routines, but included more details directly relevant to the bedtime routines.


\subsubsection{Word Counts}
% To understand the amount and quality of information contained within these submitted diary entries, we first examined patterns by their word counts, and then performed a content analysis to further investigate the type of information submitted.
In Fig.~\ref{fig:word_count} $(a)$, for each participant, we present the word counts over the week-long study, grouped by their conditions. In Fig.~\ref{fig:word_count} $(b)$, we average the word counts to the participant-level, and also present the percentage changes in word counts for each participant, between the last 3 days and the first 3 days.

Aside from one outlier in the \textit{Audio Group}, the word counts are generally comparable between the \textit{Audio Group} and the \textit{Robot Group}, with the \textit{Text Group} submitting significantly shorter entries. All three groups show a decline in the word counts over the course of the study, at roughly comparable rates.

% Topics analysis
\subsubsection{Amount of Relevant Information}
% To further investigate the \textit{quality} of the actual diary entries submitted, and how well they helped us achieve the goal of understanding the children's bedtime routines in the families, we need to go beyond word counts, and analyze the entries created. 
We present the findings of our content analysis on the diary entries in Fig.~\ref{fig:topic_count}. 
% We show the number of instances of the topic categories. found in the diary entries, aggregated at the participant-level.
% We show both the raw counts of instances, and the unique counts that only count duplicates once.
Across the two figures, we observe a higher number of activities as part of the bedtime routines being reported in the \textit{Robot Group}. Another trend that we observe is that, for some dimensions such as \textit{other activities not part of the bedtime routines}, and \textit{other details}, the \textit{Audio Group} may exhibit higher raw counts, but  similar or even lower unique counts, when compared to the \textit{Robot Group}. This reflects a tendency for entries in the \textit{Audio Group} to contain more instances of repetitive information.

In Fig.~\ref{fig:overall_info}, we present plots that are related to the level of \textit{overall information} contained within the diary entries. 
% Here we define \textit{overall information} to simply be the sum of all the (unique) counts of the various dimensions.
We see that the overall information among the three groups is much closer compared to the differences in word count, though the \textit{Text Group} is still carrying the least information on average. Looking at the trend in the level of overall information over the study duration, we see that the \textit{Text Group} was able to maintain a relatively stable level, while both the \textit{Robot Group} and the \textit{Audio Group} displayed quite a bit of variation (Fig.~\ref{fig:overall_info}~$(a)$), but that the variations in the \textit{Robot Group} were able to even out each other, essentially maintaining, on average, the same level of overall information richness between the first and last three days of the study (Fig.~\ref{fig:overall_info}~$(b)$).

\begin{figure}[tbp]
  \centering
  \includegraphics[width=0.85\linewidth]{assets/wordcount.pdf}
  \caption{Trends and analysis of \textit{Number of Words} contained in the entries}
  \label{fig:word_count}
  % \Description{Word count}
  \vspace{-12pt}
\end{figure}

\begin{figure}[bp]
  \vspace{-18pt}
  \centering
  \includegraphics[width=\linewidth]{assets/topiccount.pdf}
  \caption{Number of \textit{Information Instances} by categories}
  \label{fig:topic_count}
  % \Description{Content Analysis}
  % \vspace{-12pt}
\end{figure}


\begin{figure}[bp]
  \vspace{-18pt}
  \centering
  \includegraphics[width=0.85\linewidth]{assets/overall_info.pdf}
  \caption{Trends and analysis of \textit{Overall Information} contained in the entries}
  \label{fig:overall_info}
  % \Description{Content Analysis}
\end{figure}





\subsubsection{Subjective Self-Disclosure Reports}
% Self disclosure reported
We present the participants' self-reported self-disclosure results in Fig.~\ref{fig:post_study}. Although participants from all three conditions reported similar levels of self-disclosure in terms of depth, participants from the \textit{Robot Group} reported lower disclosure levels in terms of breadth. While there isn't a direct mapping between these questions regarding breadth and the dimensions we have analyzed for the diary entries (Fig.~\ref{fig:topic_count}), the pattern is consistent with what we are seeing in the content analysis (for the \textit{Robot Group} and the \textit{Audio Group}), where the \textit{Robot Group} covers comparable or less information on dimensions like \textit{Other Details}, but exhibit higher counts for activities directly related to the bedtime routine. 


\subsection{Usability, Ease of Learning, and Satisfaction}
\label{sec:usability}
% USE & SUS
We present the distribution of the responses in Fig.~\ref{fig:post_study}. On average, participants in the \textit{Text Group} reported the highest rating, while participants in the \textit{Robot Group} reported the lowest, and with \textit{Audio Group} in between. This pattern is consistent across the various sub-scales: usefulness, ease of use, ease of learning, satisfaction, and usability. This pattern is not unexpected, due to the simplistic nature of filling out online questionnaires. In examining the other aspects of the distribution of responses, we do notice a bimodal distribution for the ratings that is unique to the \textit{Robot Group}. Specifically, there is a higher level of user experience variance within the \textit{Robot Group}, where one subgroup rated the system highly across the sub-scales, while the other rated it low, with few participants in-between. Below we present the two main factors affecting the usability of the Diary Robot system, based on analysis of the post-study interviews with participants from the \textit{Robot Group}.

\begin{figure}[tbp]
  \centering
  \includegraphics[width=0.9\linewidth]{assets/poststudy_questions.pdf}
  \caption{Distribution of Responses to USE, SUS, and Self-disclosure}
  \label{fig:post_study}
  % \Description{Distribution of Participants' Responses to USE and SUS}
  \vspace{-12pt}
\end{figure}


\todo{maybe a separate subsection or even section, focusing on factors affecting user experiences - can move much of the current discussion to the new section too, maybe}

\subsubsection{Perceived Technical Glitches} For example, R6 reported sometimes having trouble initiating the diary activity which was frustrating for her. When we examined the system log and the recorded audio files, we found that this is usually due to inaccurate speech recognition leading the conversation awry.

% interactions such as this one shown below. In this interaction, the first sentence by the participant was not accurately processed, leading to the incorrect transcription ``We'll see ya.'' which caused an extra step of confusion. 

% \begin{enumerate}
%     \item [] \textbf{R6:} \textit{We'll see ya.}
%     \item [] \textbf{Robot:} \textit{If you want to end the conversation, you can press the bumper labelled No/Quit. Have a good night, [R6]!}
%     \item [] \textbf{R6:} \textit{It just turned off on me! Can we do a diary entry together?}
% \end{enumerate}

Note that for these technical glitches, we emphasize the word \textit{perceived} here, as they not only include true glitches, but some of the reported glitches can also be more precisely categorized as misconceptions of the expected interaction dynamic with the system, such as the user pressing the wrong button, and looking out for the wrong LED lights.

\subsubsection{Interaction Speed} Multiple participants brought up the processing time required between the questions asked as a factor that negatively influenced their experience (R1, R2, R5). R1 noted that ``...it felt very, um, like disjointed, I guess.  I think because of the processing time.'' There is, however, a second dimension to this, where the start up time of the system was also a factor. Participants generally keep the robot turned off when not in use, and have to switch it on before they can initiate the interaction. R4 described this experience: ``I wish it would've been more speedy, [...] (the start-up time was) like a minute or so, which I guess isn't that terrible but when you're used to iPads and the computer's booting up right away, sometimes I would feel frustrated ...''



% \begin{figure}[tbp]
%   \centering
%   \includegraphics[width=0.7\linewidth]{assets/compliance.pdf}
%   \caption{Compliance in Diary Entries Completion}
%   \label{fig:compliance}
%   % \Description{Compliance in Diary Entries Completion}
% \end{figure}


\subsection{Compliance}
Despite the lower self-reported usability metrics, the \textit{Robot Group} performed best in terms of compliance. Completely missed entries are rare across the conditions, with the \textit{Robot Group} being the only group having no misses at all\footnote{One participant informed us in advance that they would need to skip one day, which we did not count as a ``miss.''}. In addition, the vast majority of the entries (87.5\%) from the \textit{Robot Group} were submitted on the intended night (as opposed to sometime the next day), and without the need of a reminder. The corresponding percentage of on-time submissions are 71.4\% for the \textit{Audio Group}, and 59\% for the \textit{Text Group}. While some of the strategies discussed by the participants on sticking to the study schedule are common to all three conditions, like setting up reminders on their calendars, and mentally integrating the study activity as the last step of their bedtime routines and establishing a habit, several factors unique to the \textit{Robot Group} may have contributed to their superior compliance rate. For example, the physical presence of the robot was brought up a few times. R3 described to us ``... I think having it, um, something present in the house rather than a piece of paper, something that I look at every day when I walk past it, reminds me to do it and I feel like that was helpful.'' Similarly, R4 stated that ``I have to pass it anyway, so it would remind me, hey, don't forget to do it.'' Another factor that we did not hear bring up from the other two conditions, is the role of family members' involvement. R5 recounted that `` there were two nights that [child 1] and [child 2] had to remind me, mom we have to do Misty and I was like oh yeah.'' R1 also described getting reminders from their children, ``the kids were curious about it, so they would also remind me like, \textit{okay}, you know, \textit{go talk to the robot.  We're in bed.  Go talk to the robot.}''






\section{Discussion}
In this study, we explored the feasibility and effectiveness of using robots as interactive diaries, and found that on average, the robots were able to effectively collect the intended information. That said, careful considerations are required to support better user experiences, which could in turn also affect the quality of data collected through the process. In the discussions below, we discuss a few themes that may have had an impact on the user experiences, distilled from the interviews. We also discuss some limitations and possible extensions.

% Some of the themes we distilled from the interviews are common across the three groups, such as the desire to have some data summaries provided to \textit{the participants}, so that they could review and explore themselves how their bedtime routines have gone over the week. In the discussions below, we focus on themes that are uniquely relevant to the \textit{Robot Group}. We present recommendations and considerations for utilizing and improving upon a system such as the Diary Robot for data collection through diary studies. We also discuss some limitations of this study, and possible extensions.


\todo{add section to discuss information efficiency?}

\subsection{System and Study Design Considerations}
\subsubsection{Taking a Privacy-First Approach}
 % For the context of our study, participants generally agree that the topics of these diaries, which are about their children's bedtime routines, are not particularly sensitive or personal in nature, and 
Participants from the \textit{Text Group} and \textit{Audio Group} rarely raised any concerns about privacy, but as one can imagine, privacy is often a concern when there's a robot in your home.
% This being a research study conducted by a lab from the university was also a mitigating factor that was brought up across the three groups. 
% However, multiple participants from the \textit{Robot Group}, shared various concerns about the robot's presence within their domestic environment. 
In fact, two participants (R6, R7) mentioned that even though they were told that the camera was off, they still ``felt'' it was on. In addition, R5's partner, who was present during the equipment set up, even configured an isolated network for our system to connect to. During the study, R5 kept all the equipment unplugged or powered off, except for when she needed to interact with the Diary Robot. She described the reasoning as ``I guess there was just a little bit of wanting to have like just our regular private life.'' Privacy concerns such as these might have affected the amount of information submitted within the diary entries. R6 told us that she ``kept it very, like, short, [...] not sharing the thing that I would be uncomfortable on being out there.'' When utilizing robots as a data collection instrument in diary studies, researchers need to take a privacy-first approach. Possible plans of action include providing more transparency on the data collection and security measures~\cite{vitale2018more}, and ensuring the system is minimally invasive subject to the need of the study.


\subsubsection{Minimizing the Friction in Initializing the Interaction}
It takes a few minutes for the system to be ready for interactions, much of it involving the robot itself starting up and connecting to the controller. This is a very specific, yet frequently brought up drawback of the system (R2, R4, R6, R8). Comparing it to devices such as Alexa or Siri, R2 described his vision for a better experience: ``Like you could just say, \textit{hey, robot, I'm ready to do a diary entry}, then it would just pop on and say, \textit{OK, what do you want to talk about?}  [...] the biggest hurdle was just it wasn't always on, like Siri or something.'' Combined with the fact that we encouraged participants to complete the diary activity after the children's bedtime routines, late at night, this have exacerbated the effect of the slow start. R8 described her experience to us,``Like in the morning it was, it was easier [to set up the system] but then maybe I was more patient too because maybe I was tired at night.'' Although each system and study may require a different solution, it is clear that designing for a system that allows for a quicker start-up, or structuring a protocol that minimizes the impact of a slower start-up, shall be one of the top priorities to ensure a better user experience when repeated interactions are required.



\subsubsection{Providing a Thorough On-boarding Experience}
As detailed in section~\ref{sec:usability}, much of the complaints about usability came from the \textit{perceived} technical glitches (including both actual insufficiencies in the software, and incorrect expectations on the user's part), or a disappointment in the interaction speed (both in terms of the start-up speed, and in terms of the response speed). To properly set the expectations of the users (both in terms of the interaction flow, and the interaction speed), one approach could be through providing a more thorough on-boarding experience. In our study, to maintain comparable lengths of the in-person visits across the three conditions, we limited our instructions to the \textit{Robot Group} to a quick demo, and a five-page information pamphlet left with the participants. Participants adapted their usage patterns as they learned more about the robot, but often after already experiencing frustrations. For example, R4 told us ``... when I first started, I would turn it on and I would wait. (later on) what I would do is right before I put her to bed, I would turn it on and get it ready and then go back and do the diary faster.'' A more thorough demonstration and walk-through of the instructions and expectations of the robot's capabilities, and more concise but engaging instructions, could have potentially helped with some of these initial learning curves, and improved user experiences.

% Users, sometimes after some frustrations, adapted their usage pattern to match their experiences with the robots. For example, R4 told us ``... when I first started, I would turn it on and I would wait. [later on] what I would do is right before I put her to bed, I would turn it on and get it ready and then go back and do the diary faster.'' These little 

% instructions that are easier to read and remember, or thriving to build a more consistent and intuitive interaction flow. For example, in the context of this current project, we utilized 2 LED lights on the robot, which caused confusion for at least one participant in terms of which light was the indicator that the robot was recording. In hindsight, we could have displayed the recording indicator using both LED lights, eliminating this point of confusion.

% In terms of response time, the bulk of the time for our system was spent on the various API requests to cloud servers, for the purposes of speech-to-text, GPT-agent reasoning, and text-to-speech. While we did build in non-verbal expressions such as gaze behaviors and head tilts to simulate the robot contemplating a response, which some participants picked up on and mentioned being helpful with bridging the processing time, it seems to be insufficient in most cases. In hindsight, given the design of our study, where most of the questions the robot asked are fixed and predetermined, there are many potentials for optimizing the response time. For example, one could imagine utilizing a mix of synchronous and asynchronous responses, and doing more of the processing in the background to determine the follow-up questions once in a while. In fact, R5 even suggested something along that line: ``since most of the questions were pretty... were mostly the same, I feel like it probably could [...] not maybe process it, like, just move on to the next question and do some processing later or after a few questions?''

% The specific choice of implementation would depend on the specific circumstances, but our findings emphasize the importance of a smoothly flowing interaction, the lack of which may result in an inferior user experience, that ultimately leads to potentially inferior quality and quantity of the data collected within the diary entries.





% \subsection{Personalizing the Experience}
% Users have different preferences regarding an array of features, and allowing users to customize some of those when possible, could be another way to improve their experiences. One prominent example from this study is the voice of the robot. While some participants thought the voice was just fine, others have made comments like ``it should sound more like a robot cause it was like, a robot, but it sounded like a human. So that was weird,'' and ``Her voice is kind of odd [...] Misty seems like such a girlish name and she has like a heavy kind of smoker's voice.'' Allowing the users to choose from a pool of voices might have had an impact on improved the experience for some of these participants.




%  extensions - include media data with robot interviews
% regular structured diaries in machine readable format - paired with periodic robot interviews.

% paired with other methods

% The Diary-Interview Method
% Diary methods are typically used alongside other research methods (often questionnaires, observation, critical incident techniques, and/or interviews) in order to elicit a rich
% description of the phenomenon under study and to triangulate data. One of the most prevalent multimethod study designs involving research diaries is that of the diary-interview
% (Zimmerman & Wieder, 1977), which pairs diary keeping with follow-up interviews. A
% diary-interview study is stronger than the sum of its parts, as the interview it entails is
% grounded in and expands upon information captured in diary entries. Used conservatively,
% this follow-up interview is an opportunity to clarify or draw out selected diary entries.
% More expansively, this interview might also use diary observations as a point of departure
% for in-depth exploration. Use of the diary-interview method is discussed in the context of
% two specific studies later. These studies combine diaries and interviews in order to triangulate observations, and examine diary data in more detail through follow-up interviews.


% In the broader HCI literature, some recent studies have pointed to the exciting pro
% wei2024leveraging





\subsection{Limitations and Extensions}
% - including scale items into robot-facilitated diaries
% NOT focused on LLM. 

% limitations
% robots may also affect the usual routines being documented more
% "I usually feel completely depleted by the time we make it through bedtime and she's in her room with the light turned off and finally working on settling down. But tonight was a little bit easier due to the fact that she's really curious about the robot in the basement and she really wanted me to come and do the diary activity so that I would have a bunch of information to give her in the morning about what it was like to talk to the robot."

\subsubsection{Question Types and Diary Format} In this study, the diary method we considered are entries created based on open-ended questions, while traditional diary studies may utilize other types of data, like a series of questions based on Likert scales. We envision the \textit{Diary Robot} to be able to incorporate a limited number of these types of questions, but we also see the possibility of combining other diary formats with a \textit{Diary Robot}, where the robot would perform mini-interviews about the data collected via other formats.

\subsubsection{A Diary Study on the Robot Itself} While in-the-wild HRI studies may present a unique opportunity for utilizing the deployed robot itself for the diary study, we did not explicitly study this interesting scenario. There may be additional considerations at play when the robot is both itself the subject of the diary entries, and the entity facilitating the diary studies. Although we believe much of the high-level findings shall still apply in those cases, further investigation is required.

\subsubsection{Participants} We recruited through the university staff mailing list, and the participants were mostly the mother of middle- to upper-income households with limited racial diversity. The sample size is also limited, with eight participants for each condition. Future studies would need to be conducted with other population groups, and more participants, to assess the extent to which this method is applicable and effective in other contexts.

\subsubsection{Utilization of the Robot's Capabilities}
To be more comparable with the traditional methods, the robot's dialogue is very structured in this study. \citet{wei2024leveraging} demonstrated the potential of utilizing LLM-powered chatbots to collect self-reported data, and it would be an interesting extension to allow the robot to perform the diary studies via these more free-form conversations. In terms of multimedia and mobility capabilities, one natural extension could be a variation of the media elicitation studies described in \citet{carter2005participants}, where the robot would roam around and capture photos and videos of events and activities, and create diary entries later but using the captured media as prompts and reminders.

% While compliance for the \textit{Robot Group} has already been very high in this week-long study, if one were to perform a long-term diary study, utilizing the embodiment of the robot along with its other capabilities can be an additional means to encourage compliance. For example, the robot simply gently approaching the user with a blinking light could be more than enough to nudge the user to create the diary.

\subsubsection{Physical Embodiment} In this study, we evaluated the \textit{Diary Robot} system as a whole, against popular existing diary formats, but did not explicitly investigate the role of embodiment. While we have highlighted some advantages that might be unique to robots of physical presence, both from our results (\textit{e.g.} improved compliance) and the literature (\textit{e.g.} ability to conduct interactive interviews), and speculated on some further advantages if the physical robot's capabilities were more fully utilized, additional studies are required to understand the more nuanced mechanisms involved.


% Each extension warrants additional considerations of its own, but the general themes such as emphasizing the concerns on privacy, and ensuring a smooth and intuitive interaction, still hold as design goals to maintain the quality and quantity of the data that one will be able to collect via this method.


% \subsubsection{The Diary-Interview Method, with Robots}
% In light of the findings and discussions from this study, to make the best use of the strengths of the robotic system, one possibility could be a variation of the Diary-Interview Method~\cite{zimmerman1977diary}. Specifically, researchers could design their diary studies to have two components, with one diary component recurring more frequently as needed (\textit{nightly} in this study), and an interview component that would happen once or a few times over the course of the study. The diary component could be conducted in a similar fashion to the current study, but with mostly predetermined questions to optimize the response time. The interview component, on the other hand, would read in all the diary entries asynchronously, and perform semi-structured interviews based on the entries, to request clarifications and elaborations for a more in-depth exploration and data triangulation. While the dynamic nature of the interview will still face the same response time challenge as we have discussed, we expect the significantly lower frequency of it happening, and the higher flexibility in terms of \textit{when} it needs to happen, would greatly reduce the frustration on the participant's part regarding this aspect.

% The interview and the diary components could utilize the same robotic system, or alternatively, the diary component could also make use of other media formats such as text-input or audio recording. For example, R1 said that she ``always rather write'' when it comes to expressing herself, and allowing this flexibility to cater to the preferred method of self-expression for each participant, as long as they are machine-digestible, may prove to be an effective way of gathering more authentic and rich data of interest.









\section{Conclusion}
In this study, we explored the use of a robot in conducting diary studies as a data collection method. We developed the Diary Robot system, and carried out week-long in-home studies to evaluate its effectiveness. We compared the diary entries created from these deployments to those created from control groups utilizing existing diary methods (text-based input, and audio diaries), and found that the Diary Robot was able to effectively elicit the intended information, and efficiently collect the relevant data. Through post-study questionnaires and interviews, we further assessed users' experiences and how they could have affected the quality and quantity of the data collected. Based on those insights, we discussed some considerations when adopting this method for future studies, and noted some limitations and possible extensions.










% RONG CHANG - audio
% Nothing out of the ordinary today. Um Usually he has one meal before bed during bedtime routine. Today, he had actually three. I know I mentioned the bowl of cereal. He actually had an apple during book time. So he ate like three very, very small meals. And typically it's just the one more like 50 50 50 50. It's half the time. It's one, half the time. It's two. Um But today was three, which is a little unusual. I think it was because we were just kind of like not really doing much. So he just kind of since he wasn't on electronics wasn't really being busy. He just went up, grabbed an apple and brought it down while we were bringing the books down. So that was a little different from typical, which like I said is the one or two meals or I like to say meal. I mean, I guess you can call it snack. Um The apple was like a snack which um and that also depends on the availability of what we have for snacks. So if it's something enticing, he usually grabs it. So he likes apples usually before bed. So if we have no apples, then he probably wouldn't have had that snack. So I think that's the only thing that he did different today was he grabbed that apple. Usually, like when he grabbed the cereal today, it was, it was usually when he grabs that apple to make it that second meal. But then today he grabbed the apple before he grabbed the cereal. So that's, I guess the only thing different that happened today.




% worth2009making
% Participants often began the audio diary with short stories that were prompted by the audio diary guide. As participants got used to the recorder, and into the flow of questions, the result was longer stories diverging from the guide. Rather than approaching the diary as a totally new method, participants responded to the diary in much the same way as they did the interview; some were reflective, emotional, and confessional, while others were more concise and detail oriented (Delph-Janiurek, 2001). Most participants began the diary with a greeting, and then introduced themselves to the researcher as the listener. As the intended audience, some participants spoke to me explicitly, while others acknowledged me as a listener more indirectly by engaging me in conversation, ending phrases with, ‘you know?’ and ‘—right?’. During the data collection, one participant called to tell me she was concerned she might be doing the diary ‘wrong’ because she found it difficult to think of the diary as a monologue. I acknowledged that it can feel strange talking to a recorder on your own, and I suggested she picture a listener, which she later reported made the audio diary ‘easy’. Stylistically the audio diaries shared many of the quips and asides of the interview, and this conversational tone is one of the benefits of the audio diary, preserving ‘stream of consciousness’ thinking without the interruption that writing can sometimes be. (See work on video diaries Pink, 2007, Kindon, 2003).


% williamson2015evaluating
% The diaries produced were highly heterogeneous in terms of data length and quality. 

% \citet{li2023tell}  Negative Attitude Towards Robots Scale (NARS)

% \cite{carter2005participants}
% Media elicitation studies mitigate both of these
% concerns. In a media elicitation study, participants capture
% events, usually by taking a photo, and are asked about the
% event during an interview at a significantly later point in
% time. Thus for elicitation studies, capture is quick, and while
% the captured media still represents a subjective point-of-view,
% it has some empirical value. Barsalou posited that episodic
% memory can be improved when a person is presented with
% cues about an event such as who was involved, where it occurred or what was done just before and after the event [3].
% However, while researchers have recently begun using diary studies using photo-elicitation, it is not evident how well
% media capture these cues and to what extent media facilitate
% participant reconstruction of events. Also, different media
% types will likely evoke different reconstructions and attitudes
% towards an event, but no study has yet shown how.
